Angular analyses of exclusive $\overline{B} \to X_J \ell_1 \ell_2$ decays for spin $J \leq 4$

As an update to our previous calculation for spin $J\leq2$, we present the angular moments for exclusive $\overline{B} \to X_J \ell_1 \ell_2$, where $\ell_1$ is a charged massless lepton and $\ell_2$ is a charged or neutral massless lepton, and $X_J$ is a mesonic system with spin $J\leq4$. The expected applications include higher resonances in the $[K\pi]$ system in $\overline{B}^0 \to K^- \pi^+ \mu^- \mu^+$ at LHCb in Run~II, and in the $[\pi \pi]$ system for $ \overline{B} \to \pi \pi \ell^- \bar{\nu}_\ell$ at Belle~II. For the $J\leq2$ case, we also provide a set of consistency relations among the measured moments observables and validate them against the latest measurements from LHCb.

==> Makefile <==
# $Id: Makefile 87305 2016-02-08 13:50:32Z lafferty $
# ===============================================================================
# Purpose: simple Makefile to streamline processing latex document (just say "make" to execute)
# Author: Tomasz Skwarnicki
# Created on: 2010-09-24
# A few changes by Patrick Koppenburg on 2015-06-26
# ===============================================================================

# name of the main latex file (do not include .tex)
MAIN = main

# name of the target - change that to something descriptive, like paper-v0, Bs2PhiPhi-ANA-v1, etc...
TARGET = paper

# name of command to perform Latex (either pdflatex or latex)
LATEX = pdflatex

ifeq ($(LATEX),pdflatex)
	FIGEXT = .pdf
	MAINEXT= .pdf
	BUILDCOMMAND=rm -f $(MAIN).aux && $(LATEX) $(MAIN) && bibtex $(MAIN) && $(LATEX) $(MAIN) && $(LATEX) $(MAIN)
	BUILDCOMMANDPRL=rm -f $(MAIN)-prl.aux && $(LATEX) $(MAIN)-prl && bibtex $(MAIN)-prl && $(LATEX) $(MAIN)-prl && $(LATEX) $(MAIN)-prl
	MAKEMAINCOUNT= sed 's\#{wordcount}{false}\#{wordcount}{true}\#' main-prl.tex > main-count.tex
	BUILDCOMMANDCOUNT= $(MAKEMAINCOUNT) && rm -f $(MAIN)-count.aux && $(LATEX) $(MAIN)-count && bibtex $(MAIN)-count >/dev/null; true && $(LATEX) $(MAIN)-count && ./wordcount.sh $(MAIN)-count && rm wordcount.pdf main-count* 
else
	FIGEXT = .eps
	MAINEXT= .pdf
	BUILDCOMMAND=rm -f $(MAIN).aux && $(LATEX) $(MAIN) && bibtex $(MAIN) && $(LATEX) $(MAIN) && $(LATEX) $(MAIN) && dvips -z -o $(MAIN).ps $(MAIN) && ps2pdf $(MAIN).ps && rm -f head.tmp body.tmp
	BUILDCOMMANDPRL=rm -f $(MAIN)-prl.aux && $(LATEX) $(MAIN)-prl && bibtex $(MAIN)-prl && $(LATEX) $(MAIN)-prl && $(LATEX) $(MAIN)-prl && dvips -z -o $(MAIN)-prl.ps $(MAIN)-prl && ps2pdf $(MAIN)-prl.ps && rm -f head.tmp body.tmp
	BUILDCOMMANDCOUNT=
endif

# list of all source files
TEXSOURCES = $(wildcard *.tex) $(wildcard *.bib)
FIGSOURCES = $(wildcard figs/*$(FIGEXT))
SOURCES    = $(TEXSOURCES) $(FIGSOURCES)

# define output (could be making .ps instead)
OUTPUT = $(TARGET)$(MAINEXT)

# cp temporary main.pdf to target.
$(OUTPUT): $(MAIN)$(MAINEXT)
	cp $(MAIN)$(MAINEXT) $(OUTPUT)

# prescription how to make output (your favorite commands to process latex)
# do latex twice to make sure that all cross-references are updated 
$(MAIN)$(MAINEXT): $(SOURCES) Makefile
	$(BUILDCOMMAND)

# just so we can say "make all" without knowing the output name
all: $(OUTPUT)

# remove temporary files (good idea to say "make clean" before putting things back into repository)
.PHONY : clean
clean:
	rm -f *~ *.aux *.log *.bbl *.blg *.dvi *.tmp *.out *.blg *.bbl $(OUTPUT) $(MAIN)$(MAINEXT) $(MAIN).ps $(MAIN)-prl.ps $(MAIN)-prlNotes.bib

# remove output file
rmout: 
	rm $(OUTPUT) $(MAIN)$(MAINEXT)

# Make the PRL version
prl: 
	$(BUILDCOMMANDPRL)

# Make the PRL version
count: 
	$(BUILDCOMMANDCOUNT)
	@echo ''
	@echo 'Figures:   Add 20+150/(aspect ratio) per figure'
	@echo 'Equations: Add 16 words per row (single column) '
	@echo 'Tables:    Add 13 words plus 6.5 words per line (single column)'
	@echo 


==> babarsym.tex <==
%%%%%   Standard symbols for use in BABAR papers and BAD Notes
%%%%%
%%%%%   Revised   05/22/01 P. Dauncey     Added \hepex, etc. and clean up a bit
%%%%%   Revised   12/07/00 D. Hitlin      Added features of D. Kirkby's HEP.sty
%%%%%   Revised   07/13/00 R. Waldi       Corrected \Kbar, \Bbar ... macros
%%%%%   Revised   07/13/00 D. MacFarlane  Replaced incorrect \chic1 symbols
%%%%%   Revised   07/05/00 P. Dauncey     Added \mes, \mec, removed \O
%%%%%   Revised   07/04/00 D. MacFarlane  Added scalable version of BABAR
%%%%%   Revised   07/01/00 D. MacFarlane
%%%%%   Revised   06/21/00 D. Hitlin
%%%%%   Original  06/10/00 D. Hitlin
%%%%%   Revision of TDR and Physics Book symbol file
%%%%%

\RequirePackage{xspace}

%%%%%%%%%%%%%%%%%%%% BABAR ... THE NAME OF THE COLLABORATION %%%%

% Huge boldface
\def\hbabar{\mbox{{\huge\bf\sl B}\hspace{-0.1em}{\LARGE\bf\sl A}\hspace{-0.03em}{\huge\bf\sl B}\hspace{-0.1em}{\LARGE\bf\sl A\hspace{-0.03em}R}}}
% LARGE
\def\Lbabar{\mbox{{\LARGE\sl B}\hspace{-0.15em}{\Large\sl A}\hspace{-0.07em}{\LARGE\sl B}\hspace{-0.15em}{\Large\sl A\hspace{-0.02em}R}}}
% Large
\def\lbabar{\mbox{{\large\sl B}\hspace{-0.4em} {\normalsize\sl A}\hspace{-0.03em}{\large\sl B}\hspace{-0.4em} {\normalsize\sl A\hspace{-0.02em}R}}}
% normal size
%\def\babar{\mbox{\sl B\hspace{-0.4em} {\small\sl A}\hspace{-0.37em} \sl B\hspace{-0.4em} {\small\sl A\hspace{-0.02em}R}}}
% replace normalsize with scalable version       dbm 7/4/00
\usepackage{relsize}
\def\babar{\mbox{\slshape B\kern-0.1em{\smaller A}\kern-0.1em
    B\kern-0.1em{\smaller A\kern-0.2em R}}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%   LEPTONS   %%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\let\emi\en
\def\electron   {\ensuremath{e}\xspace}
\def\en         {\ensuremath{e^-}\xspace}   % electron negative (\em is taken)
\def\ep         {\ensuremath{e^+}\xspace}
\def\epm        {\ensuremath{e^\pm}\xspace} 
\def\epem       {\ensuremath{e^+e^-}\xspace}
\def\ee         {\ensuremath{e^-e^-}\xspace}

\def\mmu        {\ensuremath{\mu}\xspace}
\def\mup        {\ensuremath{\mu^+}\xspace}
\def\mun        {\ensuremath{\mu^-}\xspace} % muon negative (\mum is taken)
\def\mumu       {\ensuremath{\mu^+\mu^-}\xspace}
\def\mtau       {\ensuremath{\tau}\xspace}

\def\taup       {\ensuremath{\tau^+}\xspace}
\def\taum       {\ensuremath{\tau^-}\xspace}
\def\tautau     {\ensuremath{\tau^+\tau^-}\xspace}

\def\ellm       {\ensuremath{\ell^-}\xspace}
\def\ellp       {\ensuremath{\ell^+}\xspace}
\def\ellell     {\ensuremath{\ell^+ \ell^-}\xspace}

\def\nub        {\ensuremath{\overline{\nu}}\xspace}
\def\nunub      {\ensuremath{\nu{\overline{\nu}}}\xspace}
\def\nub        {\ensuremath{\overline{\nu}}\xspace}
\def\nunub      {\ensuremath{\nu{\overline{\nu}}}\xspace}
\def\nue        {\ensuremath{\nu_e}\xspace}
\def\nueb       {\ensuremath{\nub_e}\xspace}
\def\nuenueb    {\ensuremath{\nue\nueb}\xspace}
\def\num        {\ensuremath{\nu_\mu}\xspace}
\def\numb       {\ensuremath{\nub_\mu}\xspace}
\def\numnumb    {\ensuremath{\num\numb}\xspace}
\def\nut        {\ensuremath{\nu_\tau}\xspace}
\def\nutb       {\ensuremath{\nub_\tau}\xspace}
\def\nutnutb    {\ensuremath{\nut\nutb}\xspace}
\def\nul        {\ensuremath{\nu_\ell}\xspace}
\def\nulb       {\ensuremath{\nub_\ell}\xspace}
\def\nulnulb    {\ensuremath{\nul\nulb}\xspace}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%  PHOTONS  %%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\g     {\ensuremath{\gamma}\xspace}
\def\gaga  {\ensuremath{\gamma\gamma}\xspace}  %% changed from \gg, which is >>
\def\ggstar{\ensuremath{\gamma\gamma^*}\xspace}

\def\ega    {\ensuremath{e\gamma}\xspace}
\def\game   {\ensuremath{\gamma e^-}\xspace}
\def\epemg  {\ensuremath{e^+e^-\gamma}\xspace}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%  Other GAUGE BOSONS  %%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\H      {\ensuremath{H^0}\xspace}
\def\Hp     {\ensuremath{H^+}\xspace}
\def\Hm     {\ensuremath{H^-}\xspace}
\def\Hpm    {\ensuremath{H^\pm}\xspace}
\def\W      {\ensuremath{W}\xspace}
\def\Wp     {\ensuremath{W^+}\xspace}
\def\Wm     {\ensuremath{W^-}\xspace}
\def\Wpm    {\ensuremath{W^\pm}\xspace}
\def\Z      {\ensuremath{Z^0}\xspace}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%   QUARKS   %%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\q     {\ensuremath{q}\xspace}
\def\qbar  {\ensuremath{\overline q}\xspace}
\def\qqbar {\ensuremath{q\overline q}\xspace}
\def\u     {\ensuremath{u}\xspace}
\def\ubar  {\ensuremath{\overline u}\xspace}
\def\uubar {\ensuremath{u\overline u}\xspace}
\def\d     {\ensuremath{d}\xspace}
\def\dbar  {\ensuremath{\overline d}\xspace}
\def\ddbar {\ensuremath{d\overline d}\xspace}
\def\s     {\ensuremath{s}\xspace}
\def\sbar  {\ensuremath{\overline s}\xspace}
\def\ssbar {\ensuremath{s\overline s}\xspace}
\def\c     {\ensuremath{c}\xspace}
\def\cbar  {\ensuremath{\overline c}\xspace}
\def\ccbar {\ensuremath{c\overline c}\xspace}
\def\b     {\ensuremath{b}\xspace}
\def\bbar  {\ensuremath{\overline b}\xspace}
\def\bbbar {\ensuremath{b\overline b}\xspace}
\def\t     {\ensuremath{t}\xspace}
\def\tbar  {\ensuremath{\overline t}\xspace}
\def\tbar  {\ensuremath{\overline t}\xspace}
\def\ttbar {\ensuremath{t\overline t}\xspace}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%% LIGHT MESONS  %%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\piz   {\ensuremath{\pi^0}\xspace}
\def\pizs  {\ensuremath{\pi^0\mbox\,\rm{s}}\xspace}
\def\ppz   {\ensuremath{\pi^0\pi^0}\xspace}
\def\pip   {\ensuremath{\pi^+}\xspace}
\def\pim   {\ensuremath{\pi^-}\xspace}
\def\pipi  {\ensuremath{\pi^+\pi^-}\xspace}
\def\pipm  {\ensuremath{\pi^\pm}\xspace}
\def\pimp  {\ensuremath{\pi^\mp}\xspace}

\def\kaon  {\ensuremath{K}\xspace}
%%% do NOT use ensuremath here
\def\Kbar  {\kern 0.2em\overline{\kern -0.2em K}{}\xspace}
\def\Kb    {\ensuremath{\Kbar}\xspace}
\def\Kz    {\ensuremath{K^0}\xspace}
\def\Kzb   {\ensuremath{\Kbar^0}\xspace}
\def\KzKzb {\ensuremath{\Kz \kern -0.16em \Kzb}\xspace}
\def\Kp    {\ensuremath{K^+}\xspace}
\def\Km    {\ensuremath{K^-}\xspace}
\def\Kpm   {\ensuremath{K^\pm}\xspace}
\def\Kmp   {\ensuremath{K^\mp}\xspace}
\def\KpKm  {\ensuremath{\Kp \kern -0.16em \Km}\xspace}
\def\KS    {\ensuremath{K^0_{\scriptscriptstyle S}}\xspace} 
\def\KL    {\ensuremath{K^0_{\scriptscriptstyle L}}\xspace} 
\def\Kstarz  {\ensuremath{K^{*0}}\xspace}
\def\Kstarzb {\ensuremath{\Kbar^{*0}}\xspace}
\def\Kstar   {\ensuremath{K^*}\xspace}
\def\Kstarb  {\ensuremath{\Kbar^*}\xspace}
\def\Kstarp  {\ensuremath{K^{*+}}\xspace}
\def\Kstarm  {\ensuremath{K^{*-}}\xspace}
\def\Kstarpm {\ensuremath{K^{*\pm}}\xspace}
\def\Kstarmp {\ensuremath{K^{*\mp}}\xspace}

\newcommand{\etapr}{\ensuremath{\eta^{\prime}}\xspace}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%% HEAVY MESONS  %%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%% do NOT use ensuremath here
\def\Dbar    {\kern 0.2em\overline{\kern -0.2em D}{}\xspace}
\def\Db      {\ensuremath{\Dbar}\xspace}
\def\Dz      {\ensuremath{D^0}\xspace}
\def\Dzb     {\ensuremath{\Dbar^0}\xspace}
\def\DzDzb   {\ensuremath{\Dz {\kern -0.16em \Dzb}}\xspace}
\def\Dp      {\ensuremath{D^+}\xspace}
\def\Dm      {\ensuremath{D^-}\xspace}
\def\Dpm     {\ensuremath{D^\pm}\xspace}
\def\Dmp     {\ensuremath{D^\mp}\xspace}
\def\DpDm    {\ensuremath{\Dp {\kern -0.16em \Dm}}\xspace}
\def\Dstar   {\ensuremath{D^*}\xspace}
\def\Dstarb  {\ensuremath{\Dbar^*}\xspace}
\def\Dstarz  {\ensuremath{D^{*0}}\xspace}
\def\Dstarzb {\ensuremath{\Dbar^{*0}}\xspace}
\def\Dstarp  {\ensuremath{D^{*+}}\xspace}
\def\Dstarm  {\ensuremath{D^{*-}}\xspace}
\def\Dstarpm {\ensuremath{D^{*\pm}}\xspace}
\def\Dstarmp {\ensuremath{D^{*\mp}}\xspace}
\def\Ds      {\ensuremath{D^+_s}\xspace}
\def\Dsb     {\ensuremath{\Dbar^+_s}\xspace}
\def\Dss     {\ensuremath{D^*_s}\xspace}

% Obsolete
\newcommand{\dstr}{\ensuremath{\Dstar}\xspace}
\newcommand{\dstrstr}{\ensuremath{D^{**}}\xspace}
\newcommand{\dsp}{\ensuremath{\Dstarp}\xspace}
\newcommand{\dsm}{\ensuremath{\Dstarm}\xspace}
\newcommand{\dsz}{\ensuremath{\Dstarz}\xspace}


\def\B       {\ensuremath{B}\xspace}
%%% do NOT use ensuremath here
\def\Bbar    {\kern 0.18em\overline{\kern -0.18em B}{}\xspace}
\def\Bb      {\ensuremath{\Bbar}\xspace}
\def\BB      {\ensuremath{B\Bbar}\xspace} 
\def\Bz      {\ensuremath{B^0}\xspace}
\def\Bzb     {\ensuremath{\Bbar^0}\xspace}
\def\BzBzb   {\ensuremath{\Bz {\kern -0.16em \Bzb}}\xspace}
\def\Bu      {\ensuremath{B^+}\xspace}
\def\Bub     {\ensuremath{B^-}\xspace}
\def\Bp      {\ensuremath{\Bu}\xspace}
\def\Bm      {\ensuremath{\Bub}\xspace}
\def\Bpm     {\ensuremath{B^\pm}\xspace}
\def\Bmp     {\ensuremath{B^\mp}\xspace}
\def\BpBm    {\ensuremath{\Bu {\kern -0.16em \Bub}}\xspace}
\def\Bs      {\ensuremath{B_s}\xspace}
\def\Bsb     {\ensuremath{\Bbar_s}\xspace}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%% ONIA %%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\jpsi     {\ensuremath{{J\mskip -3mu/\mskip -2mu\psi\mskip 2mu}}\xspace}
\def\psitwos  {\ensuremath{\psi{(2S)}}\xspace}
\def\psiprpr  {\ensuremath{\psi(3770)}\xspace}
\def\etac     {\ensuremath{\eta_c}\xspace}
\def\chiczero {\ensuremath{\chi_{c0}}\xspace}
\def\chicone  {\ensuremath{\chi_{c1}}\xspace}
\def\chictwo  {\ensuremath{\chi_{c2}}\xspace}
\mathchardef\Upsilon="7107
\def\Y#1S{\ensuremath{\Upsilon{(#1S)}}\xspace}% no space before {...}!
\def\OneS  {\Y1S}
\def\TwoS  {\Y2S}
\def\ThreeS{\Y3S}
\def\FourS {\Y4S}
\def\FiveS {\Y5S}

%\def\chic1{\ensuremath{\chi_{c1}}}
%\def\chic2{\ensuremath{\chi_{c2}}}
%\def\chic3{\ensuremath{\chi_{c3}}}
\def\chic#1{\ensuremath{\chi_{c#1}}\xspace} % dbm


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%% BARYONS %%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\proton      {\ensuremath{p}\xspace}
\def\antiproton  {\ensuremath{\overline p}\xspace}
\def\neutron     {\ensuremath{n}\xspace}
\def\antineutron {\ensuremath{\overline n}\xspace}

\mathchardef\Deltares="7101
\mathchardef\Xi="7104
\mathchardef\Lambda="7103
\mathchardef\Sigma="7106
\mathchardef\Omega="710A

%%% do NOT use ensuremath here
\def\Deltabar{\kern 0.25em\overline{\kern -0.25em \Deltares}{}\xspace}
\def\Lbar{\kern 0.2em\overline{\kern -0.2em\Lambda\kern 0.05em}\kern-0.05em{}\xspace}
\def\Sigbar{\kern 0.2em\overline{\kern -0.2em \Sigma}{}\xspace}
\def\Xibar{\kern 0.2em\overline{\kern -0.2em \Xi}{}\xspace}
\def\Obar{\kern 0.2em\overline{\kern -0.2em \Omega}{}\xspace}
\def\Nbar{\kern 0.2em\overline{\kern -0.2em N}{}\xspace}
\def\Xb{\kern 0.2em\overline{\kern -0.2em X}{}\xspace}

\def\X {\ensuremath{X}\xspace}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%% TAU BRANCHING FRACTIONS %%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\BR         {{\ensuremath{\cal B}\xspace}}
\def\BRtauptoe  {\ensuremath{\BR(\taup \to \ep)}\xspace}
\def\BRtaumtoe  {\ensuremath{\BR(\taum \to \en)}\xspace}
\def\BRtauptomu {\ensuremath{\BR(\taup \to \mup)}\xspace}
\def\BRtaumtomu {\ensuremath{\BR(\taum \to \mun)}\xspace}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%  LIGHT HADRON DECAYS %%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\etaprepp}{\ensuremath{\etapr \to \eta \pipi}\xspace}
\newcommand{\etaprrg} {\ensuremath{\etapr \to \rho^0 \g}\xspace}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%  B DECAYS   %%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\bpsiks     {\ensuremath{\Bz \to \jpsi \KS}\xspace}
\def\bpsikst    {\ensuremath{\Bz \to \jpsi \Kstar}\xspace}
\def\bpsikl     {\ensuremath{\Bz \to \jpsi \KL}\xspace}
\def\bpsikzeropi{\ensuremath{\Bz \to \jpsi \Kstarz (\to \KL \piz)}\xspace}
\def\bpsikpluspi{\ensuremath{\Bu \to \jpsi \Kstarp (\to \KL \pip)}\xspace}
\def\bpsikpi    {\ensuremath{\Bz/\Bzb \to \jpsi (\to \mumu) \Kpm \pimp}\xspace}
\def\bupsik     {\ensuremath{\Bpm \to \jpsi (\to \mumu) \Kpm}\xspace}
\def\bpsiX      {\ensuremath{\Bz \to \jpsi \X}\xspace}

\def\Bzbtomu    {\ensuremath{\Bzb \to \mu \X}\xspace}
\def\Bzbtox     {\ensuremath{\Bzb \to \X}\xspace}
\def\Bztopipi   {\ensuremath{\Bz \to \pipi}\xspace}
\def\Bztokpi    {\ensuremath{\Bz \to \Kpm \pimp}\xspace}
\def\Bztorhopi  {\ensuremath{\Bz \to \rho^+ \pim}\xspace}
\def\Bztorhorho {\ensuremath{\Bz \to \rho \rho}\xspace}
\def\Bztokrho   {\ensuremath{\Bz \to K \rho}\xspace}
\def\Bztokstpi  {\ensuremath{\Bz \to \Kstar \pi}\xspace}
\def\Bztoapi    {\ensuremath{\Bz \to a_1 \pi}\xspace}
\def\Bztodd     {\ensuremath{\Bz \to \DpDm}\xspace}
\def\Bztodstd   {\ensuremath{\Bz \to \Dstarp \Dm}\xspace}
\def\Bztodstdst {\ensuremath{\Bz \to \Dstarp \Dstarm}\xspace}

\def\BtoDK      {\ensuremath{B \to DK}\xspace}
\def\Btodstlnu  {\ensuremath{B \to \Dstar \ell \nu}\xspace}
\def\Btodstdlnu {\ensuremath{B \to \Dstar(D) \ell \nu}\xspace}
\def\Btorholnu  {\ensuremath{B \to \rho \ell \nu}\xspace}
\def\Btopilnu   {\ensuremath{B \to \pi \ell \nu}\xspace}

\def\Btoetah    {\ensuremath{B \to \eta h}\xspace}
\def\Btoetaph   {\ensuremath{B \to \etapr h}\xspace}

\newcommand{\Betaprks}{\ensuremath{\Bz \to \etapr \KS}\xspace}
\newcommand{\Betaprkz}{\ensuremath{\Bz \to \etapr \Kz}\xspace}

\def\btosgam    {\ensuremath{b \to s \g}\xspace}
\def\btodgam    {\ensuremath{b \to d \g}\xspace}
\def\btosll     {\ensuremath{b \to s \ellell}\xspace}
\def\btosnunu   {\ensuremath{b \to s \nunub}\xspace}
\def\btosgaga   {\ensuremath{b \to s \gaga}\xspace}
\def\btosglue   {\ensuremath{b \to s g}\xspace}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%  Y(4S) DECAYS   %%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\upsbb   {\ensuremath{\FourS \to \BB}\xspace}
\def\upsbzbz {\ensuremath{\FourS \to \BzBzb}\xspace}
\def\upsbpbm {\ensuremath{\FourS \to \BpBm}\xspace}
\def\upspsikl{\ensuremath{\FourS \to (\bpsikl) (\Bzbtox)}\xspace}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%  TAU DECAYS   %%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\tauptoe    {\ensuremath{\taup \to \ep \nunub}\xspace}
\def\taumtoe    {\ensuremath{\taum \to \en \nunub}\xspace}
\def\tauptomu   {\ensuremath{\taup \to \mup \nunub}\xspace}
\def\taumtomu   {\ensuremath{\taum \to \mun \nunub}\xspace}
\def\tauptopi   {\ensuremath{\taup \to \pip \nub}\xspace}
\def\taumtopi   {\ensuremath{\taum \to \pim \nu}\xspace}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%% GAMMA-GAMMA REACTIONS %%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\ggtopi     {\ensuremath{\gaga \to \pipi}\xspace}
\def\ggtopiz    {\ensuremath{\gaga \to \ppz}\xspace}
\def\ggstox     {\ensuremath{\ggstar \to \X(1420) \to \kaon \kaon \pi}\xspace}
\def\ggstoeta   {\ensuremath{\ggstar \to \eta(550) \to \pipi \piz}\xspace}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%   KINEMATICS    %%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\ptot       {\mbox{$p$}\xspace}
%\def\pxy        {\mbox{$p_{\rm t}$}
\def\pxy        {\mbox{$p_T$}\xspace}
%\def\pt         {\mbox{$p_{\rm t}$}\xspace}
\def\pt         {\mbox{$p_T$}\xspace}
\def\mes        {\mbox{$m_{\rm ES}$}\xspace}
\def\mec        {\mbox{$m_{\rm EC}$}\xspace}
\def\DeltaE     {\mbox{$\Delta E$}\xspace}
\def\de     {\mbox{$\Delta E$}\xspace}

\def\pbcm {\ensuremath{p^*_{\Bz}}\xspace}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%   GEOMETRY    %%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\mphi       {\mbox{$\phi$}\xspace}
\def\mtheta     {\mbox{$\theta$}\xspace}
\def\ctheta     {\mbox{$\cos\theta$}\xspace}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%% ENERGY AND MOMENTUM %%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\tev}{\ensuremath{\mathrm{\,Te\kern -0.1em V}}\xspace}
\newcommand{\gev}{\ensuremath{\mathrm{\,Ge\kern -0.1em V}}\xspace}
\newcommand{\mev}{\ensuremath{\mathrm{\,Me\kern -0.1em V}}\xspace}
\newcommand{\kev}{\ensuremath{\mathrm{\,ke\kern -0.1em V}}\xspace}
\newcommand{\ev}{\ensuremath{\mathrm{\,e\kern -0.1em V}}\xspace}
\newcommand{\gevc}{\ensuremath{{\mathrm{\,Ge\kern -0.1em V\!/}c}}\xspace}
\newcommand{\mevc}{\ensuremath{{\mathrm{\,Me\kern -0.1em V\!/}c}}\xspace}
\newcommand{\gevcc}{\ensuremath{{\mathrm{\,Ge\kern -0.1em V\!/}c^2}}\xspace}
\newcommand{\mevcc}{\ensuremath{{\mathrm{\,Me\kern -0.1em V\!/}c^2}}\xspace}
%\def\ev   {\ensuremath{\rm \,e\kern -0.08em V}}
%\def\kev  {\ensuremath{\rm \,ke\kern -0.08em V}} 
%\def\mev  {\ensuremath{\rm \,Me\kern -0.08em V}} 
%\def\gev  {\ensuremath{\rm \,Ge\kern -0.08em V}} 
%\def\gevc {\ensuremath{\rm \,Ge\kern -0.08em V\!/c}} 
%\def\gevc {\ensuremath{{\rm \,Ge\kern -0.08em V\!/}c}} 
%\def\tev  {\ensuremath{\rm \,Te\kern -0.08em V}}
%\def\mevc {\ensuremath{\rm \,Me\kern -0.08em V\!/c}} 
%\def\mevc {\ensuremath{{\rm \,Me\kern -0.08em V\!/}c}} 
%\def\gevcc{\ensuremath{\rm \,Ge\kern -0.08em V\!/c^2}} 
%\def\mevcc{\ensuremath{\rm \,Me\kern -0.08em V\!/c^2}} 
%\def\gevcc{\ensuremath{{\rm \,Ge\kern -0.08em V\!/}c^2}} 
%\def\mevcc{\ensuremath{{\rm \,Me\kern -0.08em V\!/}c^2}} 


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%% DISTANCE AND AREA %%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\syin {\ensuremath{^{\prime\prime}}\xspace}
\def\inch   {\ensuremath{\rm \,in}\xspace} % \in is taken
\def\ft   {\ensuremath{\rm \,ft}\xspace}
\def\km   {\ensuremath{\rm \,km}\xspace}
\def\m    {\ensuremath{\rm \,m}\xspace}
\def\cm   {\ensuremath{\rm \,cm}\xspace}
\def\cma  {\ensuremath{{\rm \,cm}^2}\xspace}
\def\mm   {\ensuremath{\rm \,mm}\xspace}
\def\mma  {\ensuremath{{\rm \,mm}^2}\xspace}
%\def\mum  {\ensuremath{\rm \,\mum}\xspace}
\def\mum  {\ensuremath{\,\mu\rm m}\xspace}%% mu meter 
%\def\muma {\ensuremath{\rm \,\mum}^2\xspace}
\def\muma       {\ensuremath{\,\mu\rm m^2}\xspace}
\def\nm   {\ensuremath{\rm \,nm}\xspace}
\def\fm   {\ensuremath{\rm \,fm}\xspace}
\def\nm         {\ensuremath{\rm \,nm}\xspace}   %% nanometer
\def\nb         {\ensuremath{\rm \,nb}\xspace}
%
\def\barn{\ensuremath{\rm \,b}\xspace}
\def\barnhyph{\ensuremath{\rm -b}\xspace}
\def\mbarn{\ensuremath{\rm \,mb}\xspace}
\def\mbarnhyph{\ensuremath{\rm -mb}\xspace}
\def\pb {\ensuremath{\rm \,pb}\xspace}
\def\invpb {\ensuremath{\mbox{\,pb}^{-1}}\xspace}
\def\fb   {\ensuremath{\mbox{\,fb}}\xspace}
\def\invfb   {\ensuremath{\mbox{\,fb}^{-1}}\xspace}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%% TIME AND MASS  %%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\mus  {\ensuremath{\rm \,\mus}\xspace}
\def\ns   {\ensuremath{\rm \,ns}\xspace}
\def\ps   {\ensuremath{\rm \,ps}\xspace}
\def\fs   {\ensuremath{\rm \,fs}\xspace}
\def\gm   {\ensuremath{\rm \,g}\xspace}

%%\def\s{\ensuremath{\rm {\,s}}} %% second - this displays nothing  - why?
\def\sec{\ensuremath{\rm {\,s}}\xspace}       %% second - this works - jw 4/19
\def\ms         {\ensuremath{{\rm \,ms}}\xspace}     %% millisecond
\def\mus        {\ensuremath{\,\mu{\rm s}}\xspace}    %% microsecond
\def\ns         {\ensuremath{{\rm \,ns}}\xspace}      %% nanosecond
\def\ps         {\ensuremath{{\rm \,ps}}\xspace}  %% picosecond


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%   MISCELLANEOUS %%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\Xrad {\ensuremath{X_0}\xspace}
\def\NIL{\ensuremath{\lambda_{int}}\xspace}
\let\dgr\degrees


%\def\m          {\ensuremath{\rm \,m}}    %% meter
%\def\ma         {\ensuremath{\rm \,m}^2}  %% meter squared
%\def\cm         {\ensuremath{\rm \,cm}}   %% centimeter
%\def\cma        {\ensuremath{\rm \,cm}^2} %% centimeter squared
\def\cms         {\ensuremath{{\rm \,cm}^{-2} {\rm s}^{-1}}\xspace}
%\def\mm         {\ensuremath{\rm \,mm}}   %% millimeter
%\def\mma        {\ensuremath{\rm \,mm}^2} %% millimeter squared
%\def\mum        {\ensuremath{\,\mu\rm m}} %% mu meter
%\def\muma       {\ensuremath{\,\mu\rm m^2}}


\def\mic  {\ensuremath{\,\mu{\rm C}}\xspace}
\def\krad {\ensuremath{\rm \,krad}\xspace}
\def\cmc  {\ensuremath{{\rm \,cm}^3}\xspace}
\def\yr   {\ensuremath{\rm \,yr}\xspace}
\def\hr   {\ensuremath{\rm \,hr}\xspace}
\def\degc {\ensuremath{^\circ}{C}\xspace}
\def\degk {\ensuremath {\rm K}\xspace}
\def\degrees{\ensuremath{^{\circ}}\xspace}
\def\mrad{\ensuremath{\rm \,mrad}\xspace}               %% milliradian
\def\rad{\ensuremath{\rm \,rad}\xspace}
\def\mradhyph{\ensuremath{\rm -mr}\xspace}
%
\def\sx    {\ensuremath{\sigma_x}\xspace}    
\def\sy    {\ensuremath{\sigma_y}\xspace}   
\def\sz    {\ensuremath{\sigma_z}\xspace}    

%\renewcommand{\bar}[1]{\overline{#1}}  

% Some more (from Helen)
%\def\O{{\ensuremath{\cal O}}}  !!! This is a predefined LaTeX symbol !!!
\def\order{{\ensuremath{\cal O}}\xspace}
\def\L{{\ensuremath{\cal L}}\xspace}
\def\calL{{\ensuremath{\cal L}}\xspace}
%\def\S{{\ensuremath{\cal S}}}  !!! This is a predefined LaTeX symbol !!!
\def\calS{{\ensuremath{\cal S}}\xspace}
\def\calA{{\ensuremath{\cal A}}\xspace}
\def\calD{{\ensuremath{\cal D}}\xspace}
\def\calR{{\ensuremath{\cal R}}\xspace}

%% Arrows:
\def\ra                 {\ensuremath{\rightarrow}\xspace}
\def\to                 {\ensuremath{\rightarrow}\xspace}


\newcommand{\stat}{\ensuremath{\mathrm{(stat)}}\xspace}
\newcommand{\syst}{\ensuremath{\mathrm{(syst)}}\xspace}


\def\pep2{PEP-II}
\def\BF{$B$ Factory}
\def\abf {asymmetric \BF}
\def\sx    {\ensuremath{\sigma_x}\xspace}     
\def\sy    {\ensuremath{\sigma_y}\xspace}   
\def\sz    {\ensuremath{\sigma_z}\xspace}


\newcommand{\inverse}{\ensuremath{^{-1}}\xspace}
\newcommand{\dedx}{\ensuremath{\mathrm{d}\hspace{-0.1em}E/\mathrm{d}x}\xspace}
\newcommand{\chisq}{\ensuremath{\chi^2}\xspace}
\newcommand{\delm}{\ensuremath{m_{\dstr}-m_{\dz}}\xspace}
\newcommand{\lum} {\ensuremath{\mathcal{}}\xspace}

\def\gsim{{~\raise.15em\hbox{$>$}\kern-.85em
          \lower.35em\hbox{$\sim$}~}\xspace}
\def\lsim{{~\raise.15em\hbox{$<$}\kern-.85em
          \lower.35em\hbox{$\sim$}~}\xspace}



% Data processing
\def\kbytes     {\ensuremath{{\rm \,kbytes}}\xspace}
\def\kbsps      {\ensuremath{{\rm \,kbytes/s}}\xspace}
\def\kbits      {\ensuremath{{\rm \,kbits}}\xspace}
\def\kbsps      {\ensuremath{{\rm \,kbits/s}}\xspace}
\def\mbsps      {\ensuremath{{\rm \,Mbits/s}}\xspace}
\def\mbytes     {\ensuremath{{\rm \,Mbytes}}\xspace}
\def\mbps       {\ensuremath{{\rm \,Mbyte/s}}\xspace}
\def\mbsps      {\ensuremath{{\rm \,Mbytes/s}}\xspace}
\def\gbsps      {\ensuremath{{\rm \,Gbits/s}}\xspace}
\def\gbytes     {\ensuremath{{\rm \,Gbytes}}\xspace}
\def\gbsps      {\ensuremath{{\rm \,Gbytes/s}}\xspace}
\def\tbytes     {\ensuremath{{\rm \,Tbytes}}\xspace}
\def\tbpy       {\ensuremath{{\rm \,Tbytes/yr}}\xspace}
%




% QCD parameters

\newcommand{\as}{\ensuremath{\alpha_{\scriptscriptstyle S}}\xspace}
\newcommand{\MSb}{\ensuremath{\overline{\mathrm{MS}}}\xspace}
\newcommand{\LMSb}{%
  \ensuremath{\Lambda_{\overline{\scriptscriptstyle\mathrm{MS}}}}\xspace
}

% Electroweak parameters

\newcommand{\tw}{\ensuremath{\theta_{\scriptscriptstyle W}}\xspace}
\newcommand{\twb}{%
  \ensuremath{\overline{\theta}_{\scriptscriptstyle W}}\xspace
}
\newcommand{\Afb}[1]{{\ensuremath{A_{\scriptscriptstyle FB}^{#1}}}\xspace}
\newcommand{\gv}[1]{{\ensuremath{g_{\scriptscriptstyle V}^{#1}}}\xspace}
\newcommand{\ga}[1]{{\ensuremath{g_{\scriptscriptstyle A}^{#1}}}\xspace}
\newcommand{\gvb}[1]{{\ensuremath{\overline{g}_{\scriptscriptstyle V}^{#1}}}\xspace}
\newcommand{\gab}[1]{{\ensuremath{\overline{g}_{\scriptscriptstyle A}^{#1}}}\xspace}
\def\GF   {G_F} %Fermi constant

% CKM, CP violation

\def\eps{\varepsilon\xspace}
\def\epsK{\varepsilon_K\xspace}
\def\epsB{\varepsilon_B\xspace}
\def\epsp{\varepsilon^\prime_K\xspace}

\def\CP                {\ensuremath{C\!P}\xspace}
%\def\CPT               {\ensuremath{C\!P\!T}\xspace}
\def\CPT               {\ensuremath{C\!PT}\xspace} % Looks better without \!

\def\epstag  {\ensuremath{\varepsilon_{\rm tag}}\xspace}
\def\tagfac  {\ensuremath{\epstag(1-2w)^2}\xspace}

\def\rhobar {\ensuremath{\overline \rho}\xspace}
\def\etabar {\ensuremath{\overline \eta}\xspace}
%\def\paramest {\ensuremath{{\hat A}, {\hat \rho}, {\hat \eta} }}
%\def\ssparamest {\ensuremath{{\hat A}, {\hat {\sin 2 \alpha}}, 
%{\hat {\sin 2 \beta}} }}
\def\meas {\ensuremath{|V_{cb}|, |\frac{V_{ub}}{V_{cb}}|, 
|\varepsilon_K|, \Delta m_{B_d}}\xspace}

\def\Vud  {\ensuremath{|V_{ud}|}\xspace}
\def\Vcd  {\ensuremath{|V_{cd}|}\xspace}
\def\Vtd  {\ensuremath{|V_{td}|}\xspace}
\def\Vus  {\ensuremath{|V_{us}|}\xspace}
\def\Vcs  {\ensuremath{|V_{cs}|}\xspace}
\def\Vts  {\ensuremath{|V_{ts}|}\xspace}
\def\Vub  {\ensuremath{|V_{ub}|}\xspace}
\def\Vcb  {\ensuremath{|V_{cb}|}\xspace}
\def\Vtb  {\ensuremath{|V_{tb}|}\xspace}

%\def\sa{${\sin\! 2 \alpha  }$\xspace}
%\def\sb{${\sin\! 2 \beta   }$\xspace}
%\def\sg{${\sin\! 2 \gamma  }$\xspace}

% added by Gautier for tagging, tagmix, and sin2beta
\def\stwoa{\ensuremath{\sin\! 2 \alpha  }\xspace}
\def\stwob{\ensuremath{\sin\! 2 \beta   }\xspace}
\def\stwog{\ensuremath{\sin\! 2 \gamma  }\xspace}
\def\mistag{\ensuremath{w}\xspace}
\def\dilution{\ensuremath{\cal D}\xspace}
\def\deltaz{\ensuremath{{\rm \Delta}z}\xspace}
\def\deltat{\ensuremath{{\rm \Delta}t}\xspace}
\def\deltamd{\ensuremath{{\rm \Delta}m_d}\xspace}

\newcommand{\fsubd}{\ensuremath{f_D}}\xspace
\newcommand{\fds}{\ensuremath{f_{D_s}}\xspace}
\newcommand{\fsubb}{\ensuremath{f_B}\xspace}
\newcommand{\fbd}{\ensuremath{f_{B_d}}\xspace}
\newcommand{\fbs}{\ensuremath{f_{B_s}}\xspace}
\newcommand{\bsubb}{\ensuremath{B_B}\xspace}
\newcommand{\bbd}{\ensuremath{B_{B_d}}\xspace}
\newcommand{\bbs}{\ensuremath{B_{B_s}}\xspace}
\newcommand{\rgbb}{\ensuremath{\hat{B}_B}\xspace}
\newcommand{\rgbbd}{\ensuremath{\hat{B}_{B_d}}\xspace}
\newcommand{\rgbbs}{\ensuremath{\hat{B}_{B_s}}\xspace}
\newcommand{\rgbk}{\ensuremath{\hat{B}_K}\xspace}
\newcommand{\lqcd}{\ensuremath{\Lambda_{\mathrm{QCD}}}\xspace}

%\newcommand{\eqref}[1]{Eq.~(\ref{eq:#1})}
\newcommand{\secref}[1]{Section~\ref{sec:#1}}
\newcommand{\subsecref}[1]{Section~\ref{subsec:#1}}
\newcommand{\figref}[1]{Figure~\ref{fig:#1}}
\newcommand{\tabref}[1]{Table~\ref{tab:#1}}






% Journal References

% These bases are useful for ``submitted to'' when no volume is needed
\newcommand{\epjBase}        {Eur.\ Phys.\ Jour.\xspace}
\newcommand{\jprlBase}       {Phys.\ Rev.\ Lett.\xspace}
\newcommand{\jprBase}        {Phys.\ Rev.\xspace}
\newcommand{\jplBase}        {Phys.\ Lett.\xspace}
\newcommand{\nimBaseA}       {Nucl.\ Instr.\ Meth.\xspace}
\newcommand{\nimBaseB}       {Nucl.\ Instr.\ and Meth.\xspace}
\newcommand{\nimBaseC}       {Nucl.\ Instr.\ and Methods\xspace}
\newcommand{\nimBaseD}       {Nucl.\ Instrum.\ Methods\xspace}
\newcommand{\npBase}         {Nucl.\ Phys.\xspace}
\newcommand{\zpBase}         {Z.\ Phys.\xspace}


\newcommand{\apas}      [1]  {{Acta Phys.\ Austr.\ Suppl.\ {\bf #1}}}
\newcommand{\app}       [1]  {{Acta Phys.\ Polon.\ {\bf #1}}}
\newcommand{\ace}       [1]  {{Adv.\ Cry.\ Eng.\ {\bf #1}}}
\newcommand{\anp}       [1]  {{Adv.\ Nucl.\ Phys.\ {\bf #1}}}
\newcommand{\annp}      [1]  {{Ann.\ Phys.\ {\bf #1}}}
\newcommand{\araa}      [1]  {{Ann.\ Rev.\ Astr.\ Ap.\ {\bf #1}}}
\newcommand{\arnps}     [1]  {{Ann.\ Rev.\ Nucl.\ Part.\ Sci.\ {\bf #1}}}
\newcommand{\arns}      [1]  {{Ann.\ Rev.\ Nucl.\ Sci.\ {\bf #1}}}
\newcommand{\appopt}    [1]  {{Appl.\ Opt.\ {\bf #1}}}
\newcommand{\japj}      [1]  {{Astro.\ Phys.\ J.\ {\bf #1}}}
\newcommand{\baps}      [1]  {{Bull.\ Am.\ Phys.\ Soc.\ {\bf #1}}}
\newcommand{\seis}      [1]  {{Bull.\ Seismological Soc.\ of Am.\ {\bf #1}}}
\newcommand{\cmp}       [1]  {{Commun.\ Math.\ Phys.\ {\bf #1}}}
\newcommand{\cnpp}      [1]  {{Comm.\ Nucl.\ Part.\ Phys.\ {\bf #1}}}
\newcommand{\cpc}       [1]  {{Comput.\ Phys.\ Commun.\ {\bf #1}}}
\newcommand{\epj}       [1]  {\epjBase\ {\bf #1}}
%\newcommand{\epjc}      [1]  {{Eur.\ Phys.\ Jour.\ C~{\bf #1}}}
\newcommand{\epjc}      [1]  {\epjBase\ C~{\bf #1}}
\newcommand{\fizika}    [1]  {{Fizika~{\bf #1}}}
\newcommand{\fp}        [1]  {{Fortschr.\ Phys.\ {\bf #1}}}
\newcommand{\ited}      [1]  {{IEEE Trans.\ Electron.\ Devices~{\bf #1}}}
\newcommand{\itns}      [1]  {{IEEE Trans.\ Nucl.\ Sci.\ {\bf #1}}}
\newcommand{\ijqe}      [1]  {{IEEE J.\ Quantum Electron.\ {\bf #1}}}
\newcommand{\ijmp}      [1]  {{Int.\ Jour.\ Mod.\ Phys.\ {\bf #1}}}
\newcommand{\ijmpa}     [1]  {{Int.\ J.\ Mod.\ Phys.\ {\bf A{\bf #1}}}}
\newcommand{\jl}        [1]  {{JETP Lett.\ {\bf #1}}}
\newcommand{\jetp}      [1]  {{JETP~{\bf #1}}}
\newcommand{\jpg}       [1]  {{J.\ Phys.\ {\bf G{\bf #1}}}}
\newcommand{\jap}       [1]  {{J.\ Appl.\ Phys.\ {\bf #1}}}
\newcommand{\jmp}       [1]  {{J.\ Math.\ Phys.\ {\bf #1}}}
\newcommand{\jmes}      [1]  {{J.\ Micro.\ Elec.\ Sys.\ {\bf #1}}}
%\newcommand{\josa}      [1]  {{J.\ Opt.\ Soc.\ Am.\ {\bf #1}}}
\newcommand{\mpl}       [1]  {{Mod.\ Phys.\ Lett.\ {\bf #1}}}

%\newcommand{\nim}       [1]  {{Nucl.\ Instr.\ and Methods~{\bf #1}}}
\newcommand{\nim}       [1]  {\nimBaseC~{\bf #1}}
%\newcommand{\nima}      [1]  {{Nucl.\ Instr.\ Methods~{\bf A{\bf #1}}}}
\newcommand{\nima}      [1]  {\nimBaseC~A~{\bf #1}}

%\newcommand{\np}        [1]  {{Nucl.\ Phys.\ {\bf #1}}}
\newcommand{\np}        [1]  {\npBase\ {\bf #1}}
%\newcommand{\npb}       [1]  {{Nucl.\ Phys.\ {\bf B{\bf #1}}}}
\newcommand{\npb}       [1]  {\npBase\ B~{\bf #1}}
\newcommand{\npps}      [1]  {{Nucl.\ Phys.\ Proc.\ Suppl.\ {\bf #1}}}
\newcommand{\npaps}     [1]  {{Nucl.\ Phys.\ A~Proc.\ Suppl.\ {\bf #1}}}
\newcommand{\npbps}     [1]  {{Nucl.\ Phys.\ B~Proc.\ Suppl.\ {\bf #1}}}

\newcommand{\ncim}      [1]  {{Nuo.\ Cim.\ {\bf #1}}}
\newcommand{\optl}      [1]  {{Opt.\ Lett.\ {\bf #1}}}
\newcommand{\optcom}    [1]  {{Opt.\ Commun.\ {\bf #1}}}
\newcommand{\partacc}   [1]  {{Particle Acclerators~{\bf #1}}}
\newcommand{\pan}       [1]  {{Phys.\ Atom.\ Nuclei~{\bf #1}}}
\newcommand{\pflu}      [1]  {{Physics of Fluids~{\bf #1}}}
\newcommand{\ptoday}    [1]  {{Physics Today~{\bf #1}}}

%\newcommand{\jpl}       [1]  {{Phys.\ Lett.\ {\bf #1}}}      % dbm
\newcommand{\jpl}       [1]  {\jplBase\ {\bf #1}}
%\newcommand{\plb}       [1]  {{Phys.\ Lett.\ B~{\bf #1}}}   % dbm
\newcommand{\plb}       [1]  {\jplBase\ B~{\bf #1}}
\newcommand{\prep}      [1]  {{Phys.\ Rep.\ {\bf #1}}}
%\newcommand{\jprl}      [1]  {{Phys.\ Rev.\ Lett.\ {\bf #1}}} % dbm
\newcommand{\jprl}      [1]  {\jprlBase\ {\bf #1}}
%\newcommand{\pr}        [1]  {{Phys.\ Rev.\ {\bf #1}}}
\newcommand{\pr}        [1]  {\jprBase\ {\bf #1}}
%\newcommand{\jpra}      [1]  {{Phys.\ Rev.\ A~{\bf #1}}}
\newcommand{\jpra}      [1]  {\jprBase\ A~{\bf #1}}
%\newcommand{\jprd}      [1]  {{Phys.\ Rev.\ D~{\bf #1}}}
\newcommand{\jprd}      [1]  {\jprBase\ D~{\bf #1}}
%\newcommand{\jpre}      [1]  {{Phys.\ Rev.\ E~{\bf #1}}}
\newcommand{\jpre}      [1]  {\jprBase\ E~{\bf #1}}

\newcommand{\prsl}      [1]  {{Proc.\ Roy.\ Soc.\ Lond.\ {\bf #1}}}
\newcommand{\ppnp}      [1]  {{Prog.\ Part.\ Nucl.\ Phys.\ {\bf #1}}}
\newcommand{\progtp}    [1]  {{Prog.\ Th.\ Phys.\ {\bf #1}}}
\newcommand{\rpp}       [1]  {{Rep.\ Prog.\ Phys.\ {\bf #1}}}
\newcommand{\jrmp}      [1]  {{Rev.\ Mod.\ Phys.\ {\bf #1}}}  % dbm
\newcommand{\rsi}       [1]  {{Rev.\ Sci.\ Instr.\ {\bf #1}}}
\newcommand{\sci}       [1]  {{Science~{\bf #1}}}
\newcommand{\sjnp}      [1]  {{Sov.\ J.\ Nucl.\ Phys.\ {\bf #1}}}
\newcommand{\spd}       [1]  {{Sov.\ Phys.\ Dokl.\ {\bf #1}}}
\newcommand{\spu}       [1]  {{Sov.\ Phys.\ Usp.\ {\bf #1}}}
\newcommand{\tmf}       [1]  {{Teor.\ Mat.\ Fiz.\ {\bf #1}}}
\newcommand{\yf}        [1]  {{Yad.\ Fiz.\ {\bf #1}}}
%\newcommand{\zp}        [1]  {{Z.\ Phys.\ {\bf #1}}}
\newcommand{\zp}        [1]  {\zpBase\ {\bf #1}}
%\newcommand{\zpc}       [1]  {{Z.\ Phys.\ C~{\bf #1}}}
\newcommand{\zpc}       [1]  {\zpBase\ C~{\bf #1}}
\newcommand{\zpr}       [1]  {{ZhETF Pis.\ Red.\ {\bf #1}}}

\newcommand{\hepex}     [1]  {hep-ex/{#1}}
\newcommand{\hepph}     [1]  {hep-ph/{#1}}
\newcommand{\hepth}     [1]  {hep-th/{#1}}


%%%%%%%%%%%%%%%%%%%% SOFTWARE PACKAGES %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\aslund     {\mbox{\tt Aslund}\xspace}
\def\bbsim      {\mbox{\tt BBsim}\xspace}
\def\beast      {\mbox{\tt Beast}\xspace}
\def\beget      {\mbox{\tt Beget}\xspace}
\def\Bta        {\mbox{\tt Beta}\xspace}
\def\betakfit   {\mbox{\tt BetaKfit}\xspace}
\def\cornelius  {\mbox{\tt Cornelius}\xspace}
\def\evtgen     {\mbox{\tt EvtGen}\xspace}
\def\euclid     {\mbox{\tt Euclid}\xspace}
\def\fitver     {\mbox{\tt FitVer}\xspace}
\def\fluka      {\mbox{\tt Fluka}\xspace}
\def\fortran    {\mbox{\tt Fortran}\xspace}
\def\gcalor     {\mbox{\tt GCalor}\xspace}
\def\geant      {\mbox{\tt GEANT}\xspace}
\def\gheisha    {\mbox{\tt Gheisha}\xspace}
\def\hemicosm   {\mbox{\tt HemiCosm}\xspace}
\def\hepevt     {\mbox{\tt{/HepEvt/}}\xspace}
\def\jetset74   {\mbox{\tt Jetset \hspace{-0.5em}7.\hspace{-0.2em}4}\xspace}
%\def\jetset     {\mbox{\tt Jetset \hspace{-0.5em}7.\hspace{-0.2em}4}}
\def\koralb     {\mbox{\tt KoralB}\xspace}
\def\minuit     {\mbox{\tt Minuit}\xspace}
\def\objegs     {\mbox{\tt Objegs}\xspace}
\def\paw        {\mbox{\tt Paw}\xspace}
\def\root       {\mbox{\tt Root}\xspace}
\def\squaw      {\mbox{\tt Squaw}\xspace}
\def\stdhep     {\mbox{\tt StdHep}\xspace}
\def\trackerr   {\mbox{\tt TrackErr}\xspace}
\def\turtle     {\mbox{\tt Decay~Turtle}\xspace}



%-------------------------------------------------
% Add some more abbreviations - Biplab
%-------------------------------------------------
\newcommand {\vud} {V_{ud}}
\newcommand {\vus} {V_{us}}
\newcommand {\vub} {V_{ub}}
\newcommand {\vcd} {V_{cd}}
\newcommand {\vcs} {V_{cs}}
\newcommand {\vcb} {V_{cb}}
\newcommand {\vtd} {V_{td}}
\newcommand {\vts} {V_{ts}}
\newcommand {\vtb} {V_{tb}}
\newcommand {\vqb} {V_{qb}}

\newcommand {\rhoreac} {B \to \rho \ell \nu}
\newcommand {\btag} {B_{\mbox{\scriptsize tag}}}
\newcommand {\breco} {B_{\mbox{\scriptsize reco}}}
\newcommand {\bsig} {B_{\mbox{\scriptsize sig}}}
\newcommand {\bsigb} {\overline{B}_{\mbox{\scriptsize sig}}}
\newcommand {\ups} {\Upsilon(4S)}
\newcommand {\eex} {E_{\mbox{\scriptsize ex}}}
\newcommand {\mmsq} {\mbox{mm}^2}
%\newcommand {\mmsq} {m^2_{\mbox{\scriptsize miss}}}
\newcommand {\rhoz} {\rho^0}
\newcommand {\rhop} {\rho^+}
\newcommand {\ks} {K^0_S}
\newcommand {\kl} {K^0_L}
\newcommand {\etap} {\eta^'}
\newcommand {\bestups} {{\tt BestUpsilon}}
\newcommand {\cosT} {\cos(\Delta \theta_T)}
\newcommand {\thrustA} {\theta_T}
\newcommand {\pmiss} {\vec{p}_{\mbox{\scriptsize miss}} }
\newcommand {\ctl} {\cos \theta_\ell}
\newcommand {\stl} {\sin \theta_\ell}
\newcommand {\ctn} {\cos \theta_\nu}
\newcommand {\ctv} {\cos \theta_V}
\newcommand {\stv} {\sin \theta_V}
\newcommand {\thetav} {\theta_V}
\def\qsq        {\ensuremath{q^2}\xspace}
\def\thetal     {\theta_\ell} 
\def\thetaV     {\theta_V} 
\newcommand {\etal} {{\em et al.}}
\newcommand {\epsR} {\epsilon_R}
\newcommand {\thetab} {\theta_B}
\newcommand {\ctb} {\cos \theta_B}
\newcommand {\deltam} {\Delta m}
\newcommand {\xcu} {X_{\{c,u\}}}
\newcommand {\bxculnu} {\overline{B} \to \xcu \ell^- \overline{\nu}_\ell}
\newcommand {\bxlnu} {\overline{B} \to \xcu \ell^- \overline{\nu}_\ell}
\newcommand {\barnuell} {\overline{\nu}_\ell}
\newcommand {\nuell} {\nu_\ell}
\newcommand {\vckm} {V_{\mbox{\tiny CKM}}}
\newcommand {\shmax} {s^{\mbox{\tiny max}}_{\mbox{\tiny h}}}
\def\mkpi       {\ensuremath{m_{K\pi}}\xspace}


%---------------------------------------------------------
% FDIRC

\newcommand {\thc} {\theta_{\mbox{\scriptsize Ch}}}
\newcommand {\dtop} {\Delta_{\mbox{\scriptsize TOP}}}

\def\hzsq        {\ensuremath{|H_0|^2}\xspace}
\def\hpsq        {\ensuremath{|H_+|^2}\xspace}
\def\hmsq        {\ensuremath{|H_-|^2}\xspace}
\def\ssq         {\ensuremath{|S|^2}\xspace}
\def\dzsq        {\ensuremath{|D_0|^2}\xspace}
\def\dpsq        {\ensuremath{|D_+|^2}\xspace}
\def\dmsq        {\ensuremath{|D_-|^2}\xspace}
\def\hpasq        {\ensuremath{|H_\parallel|^2}\xspace}
\def\hpesq        {\ensuremath{|H_\perp|^2}\xspace}
\def\dpasq        {\ensuremath{|D_\parallel|^2}\xspace}
\def\dpesq        {\ensuremath{|D_\perp|^2}\xspace}


\def\rhzdz       {\ensuremath{Re(H_0 D^{\ast}_0)}\xspace}
\def\rshz        {\ensuremath{Re(S H_0^{ \ast})}\xspace}
\def\rhpdp       {\ensuremath{Re(H_+D^{\ast}_+)}\xspace}
\def\rhpadpa       {\ensuremath{Re(H_\parallel D^{\ast}_\parallel)}\xspace}
\def\rhpehpa       {\ensuremath{Re(H_\perp H^{\ast}_\parallel)}\xspace}
\def\rhpedpe       {\ensuremath{Re(H_\perp D^{\ast}_\perp)}\xspace}
\def\rhmdm       {\ensuremath{Re(H_- D^{ \ast}_-)}\xspace}
\def\rsdz        {\ensuremath{Re(S D_0^{ \ast})}\xspace}
\def\rhpdp       {\ensuremath{Re(H_+ D^{\ast}_+ + H_- D^{\ast}_-)}\xspace}
\def\hpdp       {\ensuremath{H_+ D^{\ast}_+ + H_- D^{\ast}_-}\xspace}
\def\rhphms      {\ensuremath{Re((H_+ + H_-)S^{\ast})}\xspace}
\def\rhphmdz     {\ensuremath{Re((H_+ + H_-)D^{\ast}_0)}\xspace}
\def\rdpdmhz     {\ensuremath{Re((D_+ + D_-)H^{\ast}_0)}\xspace}
\def\rhphmhz     {\ensuremath{Re((H_+ + H_-)S^{\ast})}\xspace}
\def\rdpdms      {\ensuremath{Re((D_+ + D_-)S^{\ast})}\xspace}
\def\rdpdmdz     {\ensuremath{Re((D_+ + D_-)D^{\ast}_0)}\xspace}
\def\rdpdm       {\ensuremath{Re(D_+ D^{ \ast}_-)}\xspace}
\def\rhphm       {\ensuremath{Re(H_+ H^{ \ast}_-)}\xspace}

\def\ihzdz       {\ensuremath{Im(H_0 D^{\ast}_0}\xspace}
\def\ishz        {\ensuremath{Im(S H_0^{ \ast})}\xspace}
\def\ihpdp       {\ensuremath{Im(H_+D^{\ast}_+)}\xspace}
\def\ihmdm       {\ensuremath{Im(H_- D^{ \ast}_-)}\xspace}
\def\isdz        {\ensuremath{Im(S D_0^{ \ast})}\xspace}
\def\ihpdp       {\ensuremath{Im(H_+ D^{\ast}_+ + H_- D^{\ast}_-)}\xspace}
\def\ihphms      {\ensuremath{Im((H_+ +H_-)S^{\ast})}\xspace}
\def\ihphmdz     {\ensuremath{Im((H_+ +H_-)D^{\ast}_0)}\xspace}
\def\idpdmhz     {\ensuremath{Im((D_+ +D_-)H^{\ast}_0)}\xspace}
\def\ihphmhz     {\ensuremath{Im((H_+ +H_-)S^{\ast})}\xspace}
\def\idpdms      {\ensuremath{Im((D_+ +D_-)S^{\ast})}\xspace}
\def\idpdmdz     {\ensuremath{Im((D_+ +D_-)D^{\ast}_0)}\xspace}

\def\qrhpede     {\ensuremath{Re(d^\dagger_\perp h_\perp)}\xspace}
% Quim's bilinears in the transversity basis

\def\qssq     {\ensuremath{|s|^2}\xspace}
\def\qhzsq     {\ensuremath{|h_0|^2}\xspace}
\def\qhpasq     {\ensuremath{|h_\parallel|^2}\xspace}
\def\qhpesq     {\ensuremath{|h_\perp|^2}\xspace}
\def\qdzsq     {\ensuremath{|d_0|^2}\xspace}
\def\qdpasq     {\ensuremath{|d_\parallel|^2}\xspace}
\def\qdpesq     {\ensuremath{|d_\perp|^2}\xspace}
\def\qrhzdz     {\ensuremath{Re(d^\dagger_0 h_0)}\xspace}
\def\qrshz     {\ensuremath{Re(h^\dagger_0 s)}\xspace}
\def\qrhpadpa     {\ensuremath{Re(d^\dagger_\parallel h_\parallel)}\xspace}
\def\qrhpedpe     {\ensuremath{Re(d^\dagger_\perp h_\perp)}\xspace}
\def\qrsdz    {\ensuremath{Re(d^\dagger_0 s)}\xspace}
\def\qrhpedpe     {\ensuremath{Re(d^\dagger_\perp h_\perp)}\xspace}
\def\qrhzdz     {\ensuremath{Re(d^\dagger_0 h_0)}\xspace}
\def\qrhpas     {\ensuremath{Re(s^\dagger h_\parallel)}\xspace}
\def\qrhpadz     {\ensuremath{Re(d^\dagger_0 h_\parallel)}\xspace}
\def\qrdpahz     {\ensuremath{Re(h^\dagger_0 d_\parallel)}\xspace}
\def\qrhpahz     {\ensuremath{Re(h^\dagger_0 h_\parallel)}\xspace}
\def\qrdpas     {\ensuremath{Re(s^\dagger d_\parallel)}\xspace}
\def\qrdpadz     {\ensuremath{Re(d^\dagger_0 d_\parallel)}\xspace}
\def\qrdpahz     {\ensuremath{Re(h^\dagger_0 d_\parallel)}\xspace}
\def\qrhpadz     {\ensuremath{Re(d^\dagger_0 h_\parallel)}\xspace}
\def\qrdpehpe     {\ensuremath{Re(h^\dagger_\perp d_\perp)}\xspace}
\def\qrhpehpa     {\ensuremath{Re(h^\dagger_\parallel h_\perp)}\xspace}
\def\qrdpedpa     {\ensuremath{Re(d^\dagger_\parallel d_\perp)}\xspace}
\def\qrhpedpa     {\ensuremath{Re(d^\dagger_\parallel h_\perp)}\xspace}
\def\qrhpadpe     {\ensuremath{Re(d^\dagger_\perp h_\parallel)}\xspace}
\def\qrhpes      {\ensuremath{Re(s^\dagger h_\perp)}\xspace}
\def\qrdpehz      {\ensuremath{Re(h^\dagger_0 d_\perp)}\xspace}
\def\qrhpedz      {\ensuremath{Re(d^\dagger_0 h_\perp)}\xspace}
\def\qrhpehz      {\ensuremath{Re(h^\dagger_0 h_\perp)}\xspace}
\def\qrdpes      {\ensuremath{Re(s^\dagger d_\perp)}\xspace}
\def\qrdpedz      {\ensuremath{Re(d^\dagger_0 d_\perp)}\xspace}



\def\qihzdz     {\ensuremath{Im(d^\dagger_0 h_0)}\xspace}
\def\qishz     {\ensuremath{Im(h^\dagger_0 s)}\xspace}
\def\qihpadpa     {\ensuremath{Im(d^\dagger_\parallel h_\parallel)}\xspace}
\def\qihpedpe     {\ensuremath{Im(d^\dagger_\perp h_\perp)}\xspace}
\def\qisdz    {\ensuremath{Im(d^\dagger_0 s)}\xspace}
\def\qihpedpe     {\ensuremath{Im(d^\dagger_\perp h_\perp)}\xspace}
\def\qihzdz     {\ensuremath{Im(d^\dagger_0 h_0)}\xspace}
\def\qihpas     {\ensuremath{Im(s^\dagger h_\parallel)}\xspace}
\def\qihpadz     {\ensuremath{Im(d^\dagger_0 h_\parallel)}\xspace}
\def\qidpahz     {\ensuremath{Im(h^\dagger_0 d_\parallel)}\xspace}
\def\qihpahz     {\ensuremath{Im(h^\dagger_0 h_\parallel)}\xspace}
\def\qidpas     {\ensuremath{Im(s^\dagger d_\parallel)}\xspace}
\def\qidpadz     {\ensuremath{Im(d^\dagger_0 d_\parallel)}\xspace}
\def\qidpahz     {\ensuremath{Im(h^\dagger_0 d_\parallel)}\xspace}
\def\qihpadz     {\ensuremath{Im(d^\dagger_0 h_\parallel)}\xspace}
\def\qidpehpe     {\ensuremath{Im(h^\dagger_\perp d_\perp)}\xspace}
\def\qihpehpa     {\ensuremath{Im(h^\dagger_\parallel h_\perp)}\xspace}
\def\qidpedpa     {\ensuremath{Im(d^\dagger_\parallel d_\perp)}\xspace}
\def\qihpedpa     {\ensuremath{Im(d^\dagger_\parallel h_\perp)}\xspace}
\def\qihpadpe     {\ensuremath{Im(d^\dagger_\perp h_\parallel)}\xspace}
\def\qihpes      {\ensuremath{Im(s^\dagger h_\perp)}\xspace}
\def\qidpehz      {\ensuremath{Im(h^\dagger_0 d_\perp)}\xspace}
\def\qihpedz      {\ensuremath{Im(d^\dagger_0 h_\perp)}\xspace}
\def\qihpehz      {\ensuremath{Im(h^\dagger_0 h_\perp)}\xspace}
\def\qidpes      {\ensuremath{Im(s^\dagger d_\perp)}\xspace}
\def\qidpedz      {\ensuremath{Im(d^\dagger_0 d_\perp)}\xspace}



\def\qhzdz     {\ensuremath{d^\dagger_0 h_0}\xspace}
\def\qshz     {\ensuremath{h^\dagger_0 s}\xspace}
\def\qhpadpa     {\ensuremath{d^\dagger_\parallel h_\parallel}\xspace}
\def\qhpedpe     {\ensuremath{d^\dagger_\perp h_\perp}\xspace}
\def\qsdz    {\ensuremath{d^\dagger_0 s}\xspace}
\def\qhpedpe     {\ensuremath{d^\dagger_\perp h_\perp}\xspace}
\def\qhzdz     {\ensuremath{d^\dagger_0 h_0}\xspace}
\def\qhpas     {\ensuremath{s^\dagger h_\parallel}\xspace}
\def\qhpadz     {\ensuremath{d^\dagger_0 h_\parallel}\xspace}
\def\qdpahz     {\ensuremath{h^\dagger_0 d_\parallel}\xspace}
\def\qhpahz     {\ensuremath{h^\dagger_0 h_\parallel}\xspace}
\def\qdpas     {\ensuremath{s^\dagger d_\parallel}\xspace}
\def\qdpadz     {\ensuremath{d^\dagger_0 d_\parallel}\xspace}
\def\qdpahz     {\ensuremath{h^\dagger_0 d_\parallel}\xspace}
\def\qhpadz     {\ensuremath{d^\dagger_0 h_\parallel}\xspace}
\def\qdpehpe     {\ensuremath{h^\dagger_\perp d_\perp}\xspace}
\def\qhpehpa     {\ensuremath{h^\dagger_\parallel h_\perp}\xspace}
\def\qdpedpa     {\ensuremath{d^\dagger_\parallel d_\perp}\xspace}
\def\qhpedpa     {\ensuremath{d^\dagger_\parallel h_\perp}\xspace}
\def\qhpadpe     {\ensuremath{d^\dagger_\perp h_\parallel}\xspace}
\def\qhpes      {\ensuremath{s^\dagger h_\perp}\xspace}
\def\qdpehz      {\ensuremath{h^\dagger_0 d_\perp}\xspace}
\def\qhpedz      {\ensuremath{d^\dagger_0 h_\perp}\xspace}
\def\qhpehz      {\ensuremath{h^\dagger_0 h_\perp}\xspace}
\def\qdpes      {\ensuremath{s^\dagger d_\perp}\xspace}
\def\qdpedz      {\ensuremath{d^\dagger_0 d_\perp}\xspace}
\def\qdpehpa      {\ensuremath{h^\dagger_\parallel d_\perp}\xspace}

\newcommand {\img} {\, Im}
\newcommand {\rel} {\, Re}

\def\lp        {\ensuremath{l_+}\xspace}
\def\lm        {\ensuremath{l_-}\xspace}
\def\mpee      {\ensuremath{m_+}\xspace}
%\def\mm        {\ensuremath{m_-}\xspace}
\def\np        {\ensuremath{n_+}\xspace}
\def\nm        {\ensuremath{n_-}\xspace}
\def\pp        {\ensuremath{p_+}\xspace}
\def\peem      {\ensuremath{p_-}\xspace}

\def\lps        {\ensuremath{l^\ast_+}\xspace}
\def\lms        {\ensuremath{l^\ast_-}\xspace}
\def\mps        {\ensuremath{m^\ast_+}\xspace}
\def\mms        {\ensuremath{m^\ast_-}\xspace}
\def\nps        {\ensuremath{n^\ast_+}\xspace}
\def\nms        {\ensuremath{n^\ast_-}\xspace}
\def\pps        {\ensuremath{p^\ast_+}\xspace}
\def\pms        {\ensuremath{p^\ast_-}\xspace}


\def\lpm        {\ensuremath{l_\pm}\xspace}
\def\mpm        {\ensuremath{m_\pm}\xspace}
\def\npm        {\ensuremath{n_\pm}\xspace}
\def\ppm        {\ensuremath{p_\pm}\xspace}

\def\lpms        {\ensuremath{l_\pm^\ast}\xspace}
\def\mpms        {\ensuremath{m_\pm^\ast}\xspace}
\def\npms        {\ensuremath{n_\pm^\ast}\xspace}
\def\ppms        {\ensuremath{p_\pm^\ast}\xspace}


\def\ezo       {\ensuremath{e_{01}}\xspace}
\def\eztw       {\ensuremath{e_{02}}\xspace}
\def\ezth       {\ensuremath{e_{03}}\xspace}
\def\ezf       {\ensuremath{e_{04}}\xspace}
\def\eoz       {\ensuremath{e_{10}}\xspace}
\def\eoo       {\ensuremath{e_{11}}\xspace}
\def\eotw       {\ensuremath{e_{12}}\xspace}
\def\eoth       {\ensuremath{e_{13}}\xspace}
\def\etwz       {\ensuremath{e_{20}}\xspace}
\def\etwo       {\ensuremath{e_{21}}\xspace}
\def\etwtw       {\ensuremath{e_{22}}\xspace}
\def\etwth       {\ensuremath{e_{23}}\xspace}
\def\ethz       {\ensuremath{e_{30}}\xspace}
\def\etho       {\ensuremath{e_{31}}\xspace}
\def\ethtw       {\ensuremath{e_{32}}\xspace}
\def\efz       {\ensuremath{e_{40}}\xspace}
\def\efo       {\ensuremath{e_{41}}\xspace}
\def\eftw       {\ensuremath{e_{42}}\xspace}
\def\efiz       {\ensuremath{e_{50}}\xspace}
\def\efio       {\ensuremath{e_{51}}\xspace}
\def\esiz       {\ensuremath{e_{60}}\xspace}
\def\esio       {\ensuremath{e_{61}}\xspace}
\def\ese       {\ensuremath{e_{7}}\xspace}
\def\ee       {\ensuremath{e_{8}}\xspace}


\def\szo       {\ensuremath{s_{01}}\xspace}
\def\sztw       {\ensuremath{s_{02}}\xspace}
\def\szth       {\ensuremath{s_{03}}\xspace}
\def\szf       {\ensuremath{s_{04}}\xspace}
\def\soo       {\ensuremath{s_{11}}\xspace}
\def\soz       {\ensuremath{s_{10}}\xspace}
\def\sotw       {\ensuremath{s_{12}}\xspace}
\def\soth       {\ensuremath{s_{13}}\xspace}
\def\stwz       {\ensuremath{s_{20}}\xspace}
\def\stwo       {\ensuremath{s_{21}}\xspace}
\def\stwtw       {\ensuremath{s_{22}}\xspace}
\def\stwth       {\ensuremath{s_{23}}\xspace}
\def\sthz       {\ensuremath{s_{30}}\xspace}
\def\stho       {\ensuremath{s_{31}}\xspace}
\def\sthtw       {\ensuremath{s_{32}}\xspace}
\def\sfz       {\ensuremath{s_{40}}\xspace}
\def\sfo       {\ensuremath{s_{41}}\xspace}
\def\sftw       {\ensuremath{s_{42}}\xspace}
\def\sfiz       {\ensuremath{s_{50}}\xspace}
\def\sfio       {\ensuremath{s_{51}}\xspace}
\def\ssi       {\ensuremath{s_{60}}\xspace}
\def\ssi       {\ensuremath{s_{61}}\xspace}
\def\sse       {\ensuremath{s_{7}}\xspace}




\def\Uze       {\ensuremath{U_{0}}\xspace}
\def\Uo       {\ensuremath{U_{1}}\xspace}
\def\Utw      {\ensuremath{U_{2}}\xspace}
\def\Uth      {\ensuremath{U_{3}}\xspace}
\def\Uf       {\ensuremath{U_{4}}\xspace}
\def\Ufi      {\ensuremath{U_{5}}\xspace}
\def\Usi      {\ensuremath{U_{6}}\xspace}
\def\Use      {\ensuremath{U_{7}}\xspace}
\def\Ue       {\ensuremath{U_{8}}\xspace}

\def\Vze       {\ensuremath{V_{0}}\xspace}
\def\Vo       {\ensuremath{V_{1}}\xspace}
\def\Vtw      {\ensuremath{V_{2}}\xspace}
\def\Vth      {\ensuremath{V_{3}}\xspace}
\def\Vf       {\ensuremath{V_{4}}\xspace}
\def\Vfi      {\ensuremath{V_{5}}\xspace}
\def\Vsi      {\ensuremath{V_{6}}\xspace}
\def\Vse      {\ensuremath{V_{7}}\xspace}
\def\Ve       {\ensuremath{V_{8}}\xspace}

\def\Kze       {\ensuremath{K_{0}}\xspace}
\def\Ko       {\ensuremath{K_{1}}\xspace}
\def\Ktw      {\ensuremath{K_{2}}\xspace}
\def\Kth      {\ensuremath{K_{3}}\xspace}
\def\Kf       {\ensuremath{K_{4}}\xspace}
\def\Kfi      {\ensuremath{K_{5}}\xspace}
\def\Ksi      {\ensuremath{K_{6}}\xspace}
\def\Kse      {\ensuremath{K_{7}}\xspace}
\def\Ke       {\ensuremath{K_{8}}\xspace}

\def\Lze       {\ensuremath{L_{0}}\xspace}
\def\Lo       {\ensuremath{L_{1}}\xspace}
\def\Ltw      {\ensuremath{L_{2}}\xspace}
\def\Lth      {\ensuremath{L_{3}}\xspace}
\def\Lf       {\ensuremath{L_{4}}\xspace}
\def\Lfi      {\ensuremath{L_{5}}\xspace}
\def\Lsi      {\ensuremath{L_{6}}\xspace}
\def\Lse      {\ensuremath{L_{7}}\xspace}
\def\Le       {\ensuremath{L_{8}}\xspace}

\def\Xze       {\ensuremath{X_{0}}\xspace}
\def\Xo       {\ensuremath{X_{1}}\xspace}
\def\Xtw      {\ensuremath{X_{2}}\xspace}
\def\Xth      {\ensuremath{X_{3}}\xspace}
\def\Xf       {\ensuremath{X_{4}}\xspace}
\def\Xfi      {\ensuremath{X_{5}}\xspace}
\def\Xsi      {\ensuremath{X_{6}}\xspace}
\def\Xse      {\ensuremath{X_{7}}\xspace}
\def\Xe       {\ensuremath{X_{8}}\xspace}

\def\Rz       {\ensuremath{R_{0}}\xspace}
\def\Ro       {\ensuremath{R_{1}}\xspace}
\def\Rtw      {\ensuremath{R_{2}}\xspace}
\def\Rth      {\ensuremath{R_{3}}\xspace}
\def\Rf       {\ensuremath{R_{4}}\xspace}
\def\Rfi      {\ensuremath{R_{5}}\xspace}
\def\Rsi      {\ensuremath{R_{6}}\xspace}
\def\Rse      {\ensuremath{R_{7}}\xspace}
\def\Rs       {\ensuremath{R_{8}}\xspace}

\def\Tz       {\ensuremath{T_{0}}\xspace}
\def\To       {\ensuremath{T_{1}}\xspace}
\def\Ttw      {\ensuremath{T_{2}}\xspace}
\def\Tth      {\ensuremath{T_{3}}\xspace}
\def\Tf       {\ensuremath{T_{4}}\xspace}
\def\Tfi      {\ensuremath{T_{5}}\xspace}
\def\Tsi      {\ensuremath{T_{6}}\xspace}
\def\Tse      {\ensuremath{T_{7}}\xspace}
\def\Ts       {\ensuremath{T_{8}}\xspace}

\def\Zz       {\ensuremath{Z_{0}}\xspace}
\def\Zo       {\ensuremath{Z_{1}}\xspace}
\def\Ztw      {\ensuremath{Z_{2}}\xspace}
\def\Zth      {\ensuremath{Z_{3}}\xspace}
\def\Zf       {\ensuremath{Z_{4}}\xspace}
\def\Zfi      {\ensuremath{Z_{5}}\xspace}
\def\Zsi      {\ensuremath{Z_{6}}\xspace}
\def\Zse      {\ensuremath{Z_{7}}\xspace}
\def\Ze       {\ensuremath{Z_{8}}\xspace}

\def\Sz       {\ensuremath{S_{0}}\xspace}
\def\So       {\ensuremath{S_{1}}\xspace}
\def\Stw      {\ensuremath{S_{2}}\xspace}
\def\Sth      {\ensuremath{S_{3}}\xspace}
\def\Sf       {\ensuremath{S_{4}}\xspace}
\def\Sfi      {\ensuremath{S_{5}}\xspace}
\def\Ssi      {\ensuremath{S_{6}}\xspace}
\def\Sse      {\ensuremath{S_{7}}\xspace}
\def\Se       {\ensuremath{S_{8}}\xspace}




